Adaptive Subspace Projection for Generative Personalization

Generative personalization often suffers from the semantic collapsing problem (SCP), where a learned personalized concept overpowers the rest of the text prompt, causing the model to ignore important contextual details. To address this, we first analyze the underlying cause, revealing that the semantic drift responsible for SCP is not random but is concentrated within a specific low-dimensional subspace. We also discover that the personalization process perturbs the embedding of the original base concept, making it an unstable reference point. Based on these insights, we introduce Test-time Embedding Adjustment with Adaptive Subspace Projection (AdaptSP), a training-free method that uses the stable, pre-trained embedding as an anchor. AdaptSP isolates the semantic drift and projects it onto the identified subspace, performing a precise adjustment that mitigates SCP while maintaining the subject identity. Our experiments show that this targeted approach significantly improves prompt fidelity and contextual alignment.

==> section/suppre.tex <==
\section{Additional experiments}

\subsection{Result on CC101 dataset}

% \vspace{-2em}

\begin{table}[h!]
    \caption{Results on CustomConcept101 dataset, tort* means tortoise plushy, teddy* means plushy teddy bear, wpot* means wooden pot. The first/\colorbox{lightgray!50} {second} metric is the $\text{CLIP-T}^{f}$/\colorbox{lightgray!50}{CLIP-I} score. The highest score is shown in \textbf{bold}, and the runner-up is \underline{underlined}.
    % The \textcolor{blue}{blue number} indicates the proposed method outperforms its baseline counterpart, while the \textcolor{red}{red number} indicates the opposite. 
    % The GAP is the average improvement over all concepts. Qualitative results are shown in Fig. \ref{fig:qualitative_comparison_celeba}.
    }
    \label{tab:cc101_results}
    \centering
    \resizebox{1\textwidth}{!}{
    \begin{tabular}{lcccccccccc}
    \toprule
    Method &  dog & cat & tort* & teddy* & chair & table & flower & wpot* & barn & Average \\
    \midrule
    % Textual Inversion  & 23.70    &  26.29    &  21.32    &  26.06    &  25.25    &  23.46    &  26.54    &  24.61   &  25.40    &  24.97  \\
    %     & \rowcolor{lightgray!50}  68.93  &  61.68  &  65.33  &  75.64  &  69.63  &  71.19  &  74.37  &  64.50 &  67.55  &  60.88  \\
    % Textual Inversion+$TEA$  & 24.23    &  26.49   & 20.97   &  27.28    &  26.11    &  23.93    &  26.89    &  25.98    &  25.69    &  25.68 \\
    %          & \rowcolor{lightgray!50}  68.48  &  59.60  &  65.20   &  71.01  &  65.73  &  66.25  &  70.56  &  62.97  &  66.72  &  59.01  \\
    % \midrule
    DreamBooth  & 20.97 & 19.21 & 25.43 & 20.9 & 21.44 & 21.57 & 20.19 & 23.14 & 24.54 & 21.93  \\
       &  \rowcolor{lightgray!50}   70.19 & 93.49 & 90.06 & 92.17 & 84.8 & 85.65 & 82.29 & 87.55 & 82.81 & \textbf{85.45} \\
    DreamBooth+$TEA$  & 21.71    &  20.10    &  25.08    &  19.65    &  23.61    &  22.97    &  23.12    &  24.99    &  26.31    &  23.06  \\
   &  \rowcolor{lightgray!50} 66.25  &  92.43  &  91.10  &  86.98   &  86.60  &  84.87  &  76.00  &  82.46  &  77.70 &   \underline{82.71} \\ \cdashlinelr{1-11}

    DreamBooth+$AdaptSP$ \\
    \quad \quad ($r_m$)  &   27.34 & 23.4 & 26.81 & 25.18 & 26.22 & 25.49 & 25.37 & 24.56 & 27.48 & \textbf{25.76}     \\
     &  \rowcolor{lightgray!50} 59.64 & 87.03 & 87.93 & 83.98 & 79.79 & 76.92 & 66.74 & 85.79 & 77.16 & 78.33 \\
    \quad \quad ($P_{\mathcal{R}}$)  &   26.16 & 21.74 & 26.22 & 24.41 & 24.8 & 23.02 & 23.98 & 23.69 & 26.21 & \underline{24.47}     \\
     &  \rowcolor{lightgray!50} 60.37 & 87.16 & 89.21 & 83.66 & 81.2 & 80.78 & 68.72 & 86.39 & 79.15 & 79.63 \\ \midrule
     
    Class Diffusion  & 26.98 & 27.41 & 29.71 & 26.08 & 25.88 & 27.1 & 25.49 & 28.12 & 27.7 & 27.16    \\
&  \rowcolor{lightgray!50} 61.17 & 82.13 & 78.97 & 86.00 & 70.53 & 64.39 & 67.31 & 73.32 & 76.22 & \textbf{73.34} \\

Class Diffusion+$TEA$  & 27.72 & 28.12 & 29.00 & 26.07 & 26.94 & 27.16 & 27.21 & 28.51 & 27.65 & \underline{27.59}     \\
        &  \rowcolor{lightgray!50} 56.44 & 77.26 & 78.87 & 77.46 & 75.56 & 60.54 & 64.87 & 60.72 & 71.27 & 69.22  \\ 
\cdashlinelr{1-11}
    Class Diffusion+$AdaptSP$ \\
    \quad \quad ($r_m$) & 27.30 & 29.06 & 29.79 & 26.18 & 25.88 & 27.10 & 26.60 & 28.82 & 28.52 & \textbf{27.69}\\
    &  \rowcolor{lightgray!50} 57.10 & 77.05 & 72.25 & 85.70 & 67.92 & 59.56 & 63.67 & 67.07 & 70.02 & 68.93  \\

    \quad \quad ($P_{\mathcal{R}}$) & 26.88 & 26.05 & 28.98 & 25.55 & 25.08 & 25.61 & 25.43 & 28.29 & 26.55 & 26.49 \\
       &  \rowcolor{lightgray!50} 60.22 & 80.89 & 78.24 & 85.82 & 69.95 & 64.02 & 64.82 & 70.61 & 74.55 & \underline{72.12}  \\ \midrule
       
    Custom Diffusion  & 26.81 & 27.65 & 29.47 & 26.27 & 25.5 & 26.32 & 25.02 & 28.0 & 26.9 & 26.88   \\
        &  \rowcolor{lightgray!50} 61.39 & 81.24 & 78.76 & 84.61 & 69.62 & 61.36 & 67.29 & 68.83 & 76.73 & 72.20 \\

Custom Diffusion+$TEA$  & 27.45    &  29.25    &  31.06    &  28.04    &  28.16    &  28.34    &  27.37    &  30.15   &  27.82    & \textbf{28.63}   \\
        &  \rowcolor{lightgray!50} 56.18  &  77.59  &  79.61  &  78.64  &  71.81  &  63.08  &  62.63  &  68.0  &  71.78  & 69.92 \\ \cdashlinelr{1-11}
    Custom Diffusion+$AdaptSP$ \\
    \quad \quad ($r_m$) & 27.42 & 29.2 & 30.22 & 26.6 & 25.53 & 26.65 & 26.44 & 28.96 & 28.6 & \underline{27.74} \\
    &  \rowcolor{lightgray!50} 57.1 & 77.04 & 73.47 & 85.09 & 67.1 & 58.06 & 63.49 & 67.76 & 69.65 & 68.75  \\

    \quad \quad ($P_{\mathcal{R}}$) & 26.58 & 25.67 & 29.37 & 25.85 & 25.37 & 25.93 & 25.4 & 28.0 & 26.32 & 26.50 \\
       &  \rowcolor{lightgray!50} 59.29 & 81.3 & 78.79 & 85.59 & 68.87 & 63.3 & 64.89 & 73.44 & 77.32 & \textbf{72.53}  \\
    \bottomrule
    \end{tabular}
    }
    % \vspace{-2em}
\end{table}

As mentioned in Section 4, we present a detailed result on the CC101 dataset in Table \ref{tab:cc101_results}.

\subsection{Visualization of generated images}

In this section, we visualize and compare images generated by different methods using the same random seed. Figures~\ref{fig:db_celebA_342}, \ref{fig:db_celebA_908}, and \ref{fig:db_celebA_181} show DreamBooth results on three CelebA concepts, while Figures~\ref{fig:db_cc101_cat}, \ref{fig:db_cc101_teddy}, and \ref{fig:db_cc101_table} show DreamBooth results on three CC101 concepts. Figures~\ref{fig:cs_celebA_342}, \ref{fig:cs_celebA_908}, and \ref{fig:cs_celebA_181} present Custom Diffusion results on the same three CelebA concepts, and Figures~\ref{fig:cs_cc101_cat}, \ref{fig:cs_cc101_teddy}, and \ref{fig:cs_cc101_table} present Custom Diffusion results on the three CC101 concepts. Class Diffusion shows similarities to Custom Diffusion, so we omit those examples here; additional qualitative comparisons are provided in the supplementary material.

Overall, AdaptSP($r_m$) represents the personalized concept $V^*$ using a single residual vector while preserving its semantic appearance, which supports our first key observation in Section 3.2. Across examples, AdaptSP improves prompt fidelity substantially, and in some cases also strengthens subject fidelity.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/db_example_celebA_342.png} 
    \caption{\textbf{DreamBooth on CelebA (concept 342):} Qualitative comparison of DreamBooth and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds for each method.}
    \label{fig:db_celebA_342}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/db_example_celebA_908.png}
    \caption{\textbf{DreamBooth on CelebA (concept 908):} Qualitative comparison of DreamBooth and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds for each method.}
    \label{fig:db_celebA_908}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/db_example_celebA_181.png}
    \caption{\textbf{DreamBooth on CelebA (concept 181):} Qualitative comparison of DreamBooth and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:db_celebA_181}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/db_example_cc101_cat.png}
    \caption{\textbf{DreamBooth on CC101 (concept cat):} Qualitative comparison of DreamBooth and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:db_cc101_cat}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/db_example_cc101_teddy.png}
    \caption{\textbf{DreamBooth on CC101 (concept teddy bear):} Qualitative comparison of DreamBooth and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:db_cc101_teddy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/db_example_cc101_table.png}
    \caption{\textbf{DreamBooth on CC101 (concept table):} Qualitative comparison of DreamBooth and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:db_cc101_table}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/cs_example_celebA_342.png}
    \caption{\textbf{Custom Diffusion on CelebA (concept 342):} Qualitative comparison of Custom Diffusion and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:cs_celebA_342}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/cs_example_celebA_908.png}
    \caption{\textbf{Custom Diffusion on CelebA (concept 908):} Qualitative comparison of Custom Diffusion and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:cs_celebA_908}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/cs_example_celebA_181.png}
    \caption{\textbf{Custom Diffusion on CelebA (concept 181):} Qualitative comparison of Custom Diffusion and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:cs_celebA_181}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/cs_example_cc101_cat.png}
    \caption{\textbf{Custom Diffusion on CC101 (concept cat):} Qualitative comparison of Custom Diffusion and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:cs_cc101_cat}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/cs_example_cc101_teddy.png}
    \caption{\textbf{Custom Diffusion on CC101 (concept teddy bear):} Qualitative comparison of Custom Diffusion and AdaptSP variants. The first row shows the training images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:cs_cc101_teddy}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/cs_example_cc101_table.png}
    \caption{\textbf{Custom Diffusion on CC101 (concept table):} Qualitative comparison of Custom Diffusion and AdaptSP variants. The first row shows the reference images. The remaining rows show generations from different prompts and random seeds.}
    \label{fig:cs_cc101_table}
\end{figure}

\section{Impact of subspace construction approach.}

To construct a meaningful semantic subspace that ensures the visual concept of interest ($V^*$ or its anchor concept $c$) is captured, the set of prompts must be chosen carefully. 
The guiding principle here is that the visual concept of interest acts as the central semantic thread common to all prompts, while the contexts are as diverse and varied as possible. 

This diversity is critical for isolating the core identity. For instance, if the prompt set frequently includes the phrase ``a man wearing glasses'', 
the resulting principal components will incorrectly learn a composite concept of ``a man with glasses'' rather than the intended, context-free concept of ``a man''. 
This is because the lack of contextual variance fails to distinguish the core identity from a recurring concept. 

Hence, we propose a set of prompts that pair the core concept ($V^*$ or $c$) with a wide range of contexts (e.g., actions, environments, artifacts, prompt length, etc.). By maximizing contextual variance, we ensure that the principal components of the embedding space capture the stable, high-variance signal of the core identity, isolating it from the lower-variance noise of individual contexts.
A set of such sample prompts is shown in Table \ref{tab:sample_prompts_subspace}.

\begin{table}[h!]
    \centering
    \caption{Sample prompts to construct the subspace. The data and prompts can be found in the supplementary material.}
    \label{tab:sample_prompts_subspace}
    \begin{tabular}{l|p{8cm}}
        \toprule
        \textbf{Set} & \textbf{Sample Sentences} \\
        \midrule
        \textbf{CelebA} & `A high-resolution photo of a \textcolor{red}{$V^*$}' \\
         & `A close-up portrait of a \textcolor{red}{$V^*$} smiling' \\
         & `A photo of a \textcolor{red}{$V^*$} looking tired but content after a long day' \\
         & `A photo of a \textcolor{red}{$V^*$} as a scientist in a laboratory, examining a petri dish' \\
         & `A watercolor painting of a \textcolor{red}{$V^*$}' \\
         & `A claymation figure of a \textcolor{red}{$V^*$}' \\
         & `A portrait of a \textcolor{red}{$V^*$} made from pressed flowers and leaves' \\
         & `A glowing, ethereal line art illustration of a \textcolor{red}{$V^*$}' \\
         & `A thermal image of a \textcolor{red}{$V^*$}' \\
        \midrule
        \textbf{CustomConcept101} & `A photo of a \textcolor{red}{$V^*$}' \\
         & `A rendering of a \textcolor{red}{$V^*$}' \\
         & `A cropped photo of a \textcolor{red}{$V^*$}' \\
         & `A portrait of a \textcolor{red}{$V^*$}' \\
         & `A close-up shot of a \textcolor{red}{$V^*$}' \\
         & `\textcolor{red}{$V^*$} next to a rustic wooden cabin' \\
         & `\textcolor{red}{$V^*$} covered in vines and moss' \\
         & `\textcolor{red}{$V^*$} in front of a glowing full moon' \\
         & `A cozy cabin with \textcolor{red}{$V^*$} sitting by the door' \\
        \bottomrule
    \end{tabular}
    % \vspace{-2em}
\end{table}

% \subsection{Problem of Subject Fidelity Metrics} 

% \subsection{Anchor choice}

% Compare $\tau_{\phi}(\lfloor p_i, c \lfloor)$ vs $\tau_{\phi_0}(\lfloor p_i, c \lfloor)$

% \subsection{}

% Idea: measure similarity between the secondary entity crop (how to automatically crop it?) and the reference set (sks man). If it’s too high, leakage is happening.

% proof for claim: Cross-class prompts: “kid”, “woman”, “old man”, etc. Track how much the output shifts toward the subject identity.

% Diversity metrics across multiple seeds and contexts: intra-set LPIPS, or DINO feature variance, or pairwise distance.
